On Tightness of Tsaknakis-Spirakis Descent Methods for Approximate Nash Equilibria

This article explores the minimum approximation ratio for Nash equilibrium in bi-matrix games, focusing on the Tsaknakis and Spirakis (TS) methods. The previous SOTA, TS algorithm, achieved an approximation ratio of 0.3393, but efforts to improve the analysis of the TS algorithm have been unsuccessful. This work demonstrates that the bound of 0.3393 is tight for the TS algorithm and presents a theoretical worst-case analysis. A condition for identifying tight instances is provided, along with a generator. While most generated instances are unstable, indicating potential improvements, stable instances exist where perturbations cannot enhance the 0.3393 bound. Other approximate algorithms, such as regret-matching and fictitious play, achieve better ratios on these instances. The generated instances can serve as benchmarks for approximate Nash equilibrium algorithms. The article also mentions progress in the TS algorithm, achieving an approximation ratio of 1/3, which can be further studied using the presented techniques.

==> Sections/DistPropOfGenerator.tex <==
\section{Distribution Properties of Tight Instance Generator}\label{sec:dist-prop-of-tight-instance}

In this section we analyze the conditions on $R,C$ for the tight instance to be PSU and DSU.

Firstly, []%reference TS
that the problem
$\max_{\rho,w,z} \min_{x',y'} T(x,y,x',y',\rho,w,z)$ can be rewritten as the following minimax problem:
$$\max_{\rho,w,z} \min_{x',y'}\begin{bmatrix}\rho w^T&(1-\rho)z^T\end{bmatrix}G(x,y,R,C)\begin{bmatrix}y'\\x'\end{bmatrix}, $$
where\begin{enumerate}[label=\alph*)]
    \item $\begin{bmatrix}\rho w\\(1-\rho)z\end{bmatrix}\in \Delta_{m+n}$, $\supp(w)\subseteq S_R(y)$, $\supp(z)\subseteq S_C(x)$
    \item $(x',y')\in \Delta_m\times\Delta_n$
    \item $G(x,y,R,C)$ is the following $(m+n)\times (m+n)$ matrix:
    $$G(x,y,R,C)=\begin{bmatrix}R-e_mx^TR &-e_my^TR^T+e_mx^TRye_m^T\\
    -e_nx^TC+e_nx^TCye_n^T &C^T-e_ny^TC^T\end{bmatrix}$$
\end{enumerate}

Let $S_u=S_R(y)\cup\{m+j:j\in S_C(x)\}$, which is the positions in $\begin{bmatrix}\rho w\\(1-\rho)z\end{bmatrix}$ that may be positive. When $x,y,R,C$ is given, $S_u$ is fixed, and there is a trivial one-to-one mapping from $\begin{bmatrix}\rho w\\(1-\rho)z\end{bmatrix}$ to a vector $u\in\Delta_{|S_u|}$ by removing all the entries not in $S_u$.

We can express this problem in the form of standard two-person zero-sum matrix game equivalently, by removing the rows of $G$ \footnote{we omit the parameters $(x,y,R,C)$ for brevity.} not in $S_u$, and mapping $(x',y')$ into $\Delta_{mn}$.

Let $\phi(x',y')$ maps $(x',y')\in\Delta_m\times\Delta_n$ to $v\in\Delta_{mn}$, where $v_{i,j}:=x_iy_j$.\footnote{for convenience, we use $v_{i,j}$ to denote $v_{(i-1)n+j}$}
It's easy to check that $\forall i, \sum_j v_{i,j}=x'_i$, and $\forall j, \sum_{i}v_{i,j}=y'_j$.

Given any $v\in\Delta_{mn}$, we can map it to $(x',y')\in\Delta_m\times\Delta_n$, where $\forall i=1,\cdots,m,\ x'_i=\sum_{j=1}^n v_{i,j}$, and $\forall j=1,\cdots,n,\ y'_j=\sum_{i=1}^mv_{i,j}$. For convenience we denote this mapping by $(x',y')=\phi^{-1}(v)$. Note that $\forall (x',y')\in\Delta_m\times\Delta_n$, $\phi^{-1}(\phi(x',y'))=(x',y')$.

Then we construct a $(m+n)\times(mn)$ payoff matrix $A(x,y,R,C)$, let \[A_{k,(i-1)n+j}=G_{k,n+i}+G_{k,j},\] for all $k\in\{1,\cdots,m+n\},i\in\{1,\cdots,m\},j\in\{1,\cdots,n\}$.
Note that when $x,y$ is fixed, every entry of $G(x,y,R,C)$ is a linear combination of some entries of $R$ and $C$, and this still holds for every entry of $A(x,y,R,C)$.

Let $G_{S_u}$ and $A_{S_u}$ denote respectively the submatrix of $A$ and $G$ containing the rows in $S_u$. Now we prove that the earlier minimax problem is equivalent with $$\max_{u\in\Delta_{|S_u|}} \min_{v\in\Delta_{mn}}u^TA_{S_u}v.$$

\begin{lemma}
The two minimax problems have the same optimal value:
$$\max_{\rho,w,z} \min_{x',y'}\begin{bmatrix}\rho w^T&(1-\rho)z^T\end{bmatrix}G\begin{bmatrix}y'\\x'\end{bmatrix}=\max_{u\in\Delta_{|S_u|}} \min_{v\in\Delta_{mn}}u^TA_{S_u}v.$$ Moreover, any optimal solution of $(\rho,w,z)$ or $(x',y')$ in the former problem corresponds to an  optimal solution of $u$ or $v$ in the latter problem respectively, and vice versa.
\end{lemma}
\begin{proof}
For any $v\in\Delta_{mn}$, if $(x',y')=\phi^{-1}(v)$, then $\forall k\in\{1,\cdots,m+n\}$,
$$(Av)_k=\sum_{i=1}^m\sum_{j=1}^nv_{(i-1)n+j}A_{k,(i-1)n+j}=\sum_{i=1}^mG_{k,n+i}\sum_{j=1}^nv_{i,j}+\sum_{j=1}^nG_{k,j}\sum_{i=1}^mv_{i,j}=\left(G\begin{bmatrix}y'\\x'\end{bmatrix}\right)_k,$$
therefore $Av=G\begin{bmatrix}y'\\x'\end{bmatrix}$ holds whenever $(x',y')=\phi^{-1}(v)$.

$\forall u\in\Delta_{|S_u|}$, $\forall (x',y')\in \Delta_m\times\Delta_n$, as $\phi^{-1}(\phi(x',y'))=(x',y')$, we have $G\begin{bmatrix}y'\\x'\end{bmatrix}=A\phi(x',y')$, and $G_{S_u}\begin{bmatrix}y'\\x'\end{bmatrix}=A_{S_u}\phi(x',y')$, so  $u^TG_{S_u}\begin{bmatrix}y'\\x'\end{bmatrix}=u^TA_{S_u}\phi(x',y')$. On the other hand $\forall v\in\Delta_{mn}$, let $(x',y')=\phi^{-1}(v)$, then $u^TA_{S_u}v=u^TG_{S_u}\begin{bmatrix}y'\\x'\end{bmatrix}$, so we have
$$\max_u\min_{x',y'}u^TG_{S_u}\begin{bmatrix}y'\\x'\end{bmatrix}=\max_u\min_{v}u^TA_{S_u}v.$$

Obviously $\phi$ converts an optimal solution of $(x',y')$ into an optimal solution of $v$, and $\phi^{-1}$ does the opposite.

It is also equivalent to convert $\begin{bmatrix}\rho w\\(1-\rho)z\end{bmatrix}$
and $u$ to each other by removing or adding the entries not in $S_u$, as those entries must be zero. Hence we have
$$\max_{\rho,w,z} \min_{x',y'}\begin{bmatrix}\rho w^T&(1-\rho)z^T\end{bmatrix}G\begin{bmatrix}y'\\x'\end{bmatrix}=\max_u\min_{x',y'}u^TG_{S_u}\begin{bmatrix}y'\\x'\end{bmatrix}=\max_{u\in\Delta_{|S_u|}} \min_{v\in\Delta_{mn}}u^TA_{S_u}v.$$

[]%reference:SOLUTIONS OF FINITE TWO-PERSON GAMES
gives a sufficient and necessary condition for a two-person zero-sum game to have certain given optimal strategy sets.



\end{proof}

